On Khovanov's cobordism theory for su(3) knot homology

We reconsider the su(3) link homology theory defined by Khovanov in math.QA/0304375 and generalized by Mackaay and Vaz in math.GT/0603307. With some slight modifications, we describe the theory as a map from the planar algebra of tangles to a planar algebra of (complexes of) `cobordisms with seams' (actually, a `canopolis'), making it local in the sense of Bar-Natan's local su(2) theory of math.GT/0410495. We show that this `seamed cobordism canopolis' decategorifies to give precisely what you'd both hope for and expect: Kuperberg's su(3) spider defined in q-alg/9712003. We conjecture an answer to an even more interesting question about the decategorification of the Karoubi envelope of our cobordism theory. Finally, we describe how the theory is actually completely computable, and give a detailed calculation of the su(3) homology of the (2,n) torus knots.

==> article/algebraic_invariant.tex <==
\subsection{The algebraic invariant for tangles}
It's relatively straightforward to describe the `algebraic'
$\su{3}$ invariant for tangles, following the usual correspondence
between Bar-Natan's invariant for tangles in \cite{MR2174270}, and
Khovanov's, which makes use of the rings he calls `$H_n$' in
\cite{MR1928174}. However, since this correspondence isn't as well
known as it might be, we'll spell it out again in the $\su{3}$ case.

Fix for now some boundary $\bdy$. Each diagram $D \in \Cob{3}_\bdy$
gives a representation $\rho_D$ of the category $\Cob{3}_\bdy$ in
$\ZMod$, via\footnote{This isn't quite the same as the `tautological functor' construction in \cite{MR2174270}; it's a slice of $\operatorname{Hom}$ in the opposite direction.}
\begin{align*}
 \rho_D : D' & \mapsto \Hom{}{D}{D'} \\
 \rho_D : (\varphi: D' \To D'') & \mapsto
   \left\{\begin{aligned}
    \Hom{}{D}{D'} & \To \Hom{}{D}{D''} \\
    v             & \mapsto \varphi \compose v
   \end{aligned}\right.
\end{align*}

A complex $C^\bullet$ in $\Kom{\Cob{3}_\bdy}$ gives a representation
$\rho_{C^\bullet}$ in $\Kom{\ZMod}$ in the same way.

Almost trivially, $\Cob{3}$ is Morita equivalent to
$\Cob{3}^\text{ne}$, the full subcategory of non-elliptic diagrams.
You might thus think of the representation of $\Cob{3}$ associated
to $D$ first as a representation of $\Cob{3}^\text{ne}$, then as
just a single module:
$$\DirectSum_{\text{$D'$ non-elliptic}} \Hom{}{D}{D'}$$
along with a right action of the ring
$$H_\bdy = \DirectSum_{\text{$D_1, D_2$ non-elliptic}} \Hom{}{D_1}{D_2},$$
which is just the direct sum of all the $\operatorname{Hom}$ spaces
in the category. We wanted to pass to the Morita equivalent
$\Cob{3}^\text{ne}$ before doing this, so everything is
finite-dimensional. The same holds for complexes; associated to
$C^\bullet$ we obtain a complex of $H_\bdy$ modules.

Thus, starting with a tangle, we construct our `geometric' complex,
then apply this construction to produce an `algebraic' complex, a complex of $H_\bdy$-modules. It
turns out, although we'll omit the details, that this complex of
modules still lives in a planar algebra. We'll see a restricted case
of this in a moment. This complex is not, however, the $\su{3}$
analogue of Khovanov's construction of an algebraic tangle
invariant. To produce that, we need to pick a decomposition of the boundary
of our tangle into `top' and `bottom' pieces, $\bdy = \bdy_t
\cup \bdy_b$, and we'll abandon our aspirations of producing an
invariant living in a planar algebra, but only look for a rule for
composing the invariants associated to two tangles `top to bottom'.

Instead of looking for a representation of $\Cob{3}_\bdy$ associated
to the complex, we'll restrict our attention to the full subcategory
$\Cob{3}_{\bdy_t} \times \Cob{3}_{\bdy_b}$, or in fact to the
non-elliptic part of that, $\Cob{3}^{\text{ne}}_{\bdy_t} \times
\Cob{3}^{\text{ne}}_{\bdy_b}$. We can think of the representation of
$\Cob{3}_{\bdy_t} \times \Cob{3}_{\bdy_b}$ associated to a diagram
$D$ as being a $\Cob{3}_{\bdy_t}-\Cob{3}_{\bdy_b}^{\text{op}}$
bimodule. Alternatively, thinking in terms of the ring of all morphisms, to a diagram $D$ we can associate the
module
$$\mathcal{F}(D) = \DirectSum_{\substack{D_t \in \bdy_t, D_b \in \bdy_b \\ \text{non-elliptic}}} \Hom{}{D}{D_t \sqcup D_b}$$
and remember the action of the ring $H_{(\bdy_t,\bdy_b)}$ which is
just isomorphic to $H_{\bdy_t} \tensor H_{\bdy_b}$. Actually, this
isomorphism isn't trivial; it depends fundamentally on the topology
of foams, and the particular relations, neck cutting, tube and
rocket, we've imposed. We can think of this module as a
$H_{\bdy_t}-H_{\bdy_b}^{\text{op}}$ bimodule, if we prefer. As
usual, the same sort of construction works for complexes; we obtain
a complex of bimodules.

We now ask how we can produce $\rho_{D_1 \cup_{\bdy_m} D_2}$, for diagrams
$D_1 \in \Cob{3}_{\bdy_t \cup \bdy_m}$ and $D_2 \in \Cob{3}_{\bdy_m
\cup \bdy_b}$. We claim that
\begin{align}
\label{eq:gluing-rule}
  \rho_{D_1 \cup_{\bdy_m} D_2}(D_t \sqcup D_b) & = \Hom{}{D_1 \cup D_2}{D_t \sqcup D_b} \\
    \notag
    & = \frac{\DirectSum_{D_m \in \Cob{3}_{\bdy_m}} \Hom{}{D_1}{D_t \sqcup D_m} \tensor \Hom{}{D_2}{\mirror{D_m} \sqcup D_b}}
           {\left(v \tensor ((f \sqcup \Id_{D_b})\compose w) = ((\Id_{D_t} \sqcup \mirror{f}) \compose v) \tensor w\right)}
\end{align}
Here $f$ is an arbitrary morphism $f:D_m \To D_m'$, with $D_m$ and
$D_m'$ both in $\Cob{3}_{\bdy_m}$, $v \in \Hom{}{D_1}{D_t \sqcup D_m'}$ and $w \in \Hom{}{D_2}{\mirror{D_m} \sqcup D_b}$.
There's an obvious map from the direct sum in the numerator of the right
hand side back to the left side, given, on elementary tensors,
simply by gluing together the cobordisms along $D_m$. We claim that
the kernel of this map is exactly the span of the relations given above, and
that every element of the left side appears this way, simply because
we can cut up a morphism on the left side into two appropriate
pieces, for some diagram $D_m$. See \cite{kw:tqft} for the details of
this sort of argument.

Thinking of $\rho_{D_1 \cup D_2}$ as a
$\Cob{3}_{\bdy_t}-\Cob{3}_{\bdy_b}^{\text{op}}$ bimodule, Equation
\ref{eq:gluing-rule} simply says
\begin{equation*}
\rho_{D_1 \cup D_2} = \rho_{D_1} \Tensor_{\Cob{3}_{\bdy_m}} \rho_{D_2}.
\end{equation*}
Translated into the langauge of the ring of morphisms, this says
\begin{equation*}
\rho_{D_1 \cup D_2} = \rho_{D_1} \Tensor_{H_{\bdy_m}} \rho_{D_2},
\end{equation*}
as $H_{\bdy_t}-H_{\bdy_b}^{\text{op}}$ bimodules. That is, the
bimodule invariant associated to two diagrams stacked together is
just the tensor product over $H_{\bdy_m}$ of the individual bimodule
invariants. Stepping up from bimodules associated to spider diagrams
to complexes of bimodules associated to tangles, we have exactly the
statement corresponding to the $\su{2}$ result described by
Khovanov in \cite{MR1928174,MR2171235}.


==> todolist.tex <==
%auto-ignore
%this ensures the arxiv doesn't try to start TeXing here.
\section*{todo list}
\begin{itemize}
\item proofread for language
\item email drafts
\item arXiv
\item decide where to submit
\item submit!
\end{itemize}


==> xkeyval.tex <==
%auto-ignore
%this ensures the arxiv doesn't try to start TeXing here.
%auto-ignore
%this ensures the arxiv doesn't try to start TeXing here.
%%
%% This is file `xkeyval.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% xkeyval.dtx  (with options: `xkvtex')
%%
%% ---------------------------------------
%% Copyright (C) 2004-2005 Hendri Adriaens
%% ---------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2003/12/01 or later.
%%
%% This work has the LPPL maintenance status "maintained".
%%
%% This Current Maintainer of this work is Hendri Adriaens.
%%
%% This work consists of the file xkeyval.dtx and derived files
%% keyval.tex, xkvtxhdr.tex, xkeyval.sty, xkeyval.tex, xkvview.sty,
%% xkvltxp.sty, pst-xkey.tex, pst-xkey.sty, xkveca.cls, xkvecb.cls,
%% xkvesa.sty, xkvesb.sty, xkvesc.sty, xkvex1.tex, xkvex2.tex,
%% xkvex3.tex and xkvex4.tex.
%%
%% The following files constitute the xkeyval bundle and must be
%% distributed as a whole: readme, xkeyval.pdf, keyval.tex,
%% pst-xkey.sty, pst-xkey.tex, xkeyval.sty, xkeyval.tex, xkvview.sty,
%% xkvltxp.sty, xkvtxhdr.tex, pst-xkey.dtx and xkeyval.dtx.
%%
\csname XKeyValLoaded\endcsname
\let\XKeyValLoaded\endinput
\edef\XKVcatcodes{%
  \catcode`\noexpand\@\the\catcode`\@\relax
  \catcode`\noexpand\=\the\catcode`\=\relax
  \catcode`\noexpand\,\the\catcode`\,\relax
  \catcode`\noexpand\:\the\catcode`\:\relax
  \let\noexpand\XKVcatcodes\relax
}
\catcode`\@11\relax
\catcode`\=12\relax
\catcode`\,12\relax
\catcode`\:12\relax
\newtoks\XKV@toks
\newcount\XKV@depth
\newif\ifXKV@st
\newif\ifXKV@sg
\newif\ifXKV@pl
\newif\ifXKV@knf
\newif\ifXKV@rkv
\newif\ifXKV@inpox
\newif\ifXKV@preset
\let\XKV@rm\@empty
\ifx\ProvidesFile\@undefined
  \message{2005/11/25 v2.5e key=value parser (HA)}
  \input xkvtxhdr
\else
  \ProvidesFile{xkeyval.tex}[2005/11/25 v2.5e key=value parser (HA)]
  \@addtofilelist{xkeyval.tex}
\fi
\long\def\@firstoftwo#1#2{#1}
\long\def\@secondoftwo#1#2{#2}
\long\def\XKV@afterfi#1\fi{\fi#1}
\long\def\XKV@afterelsefi#1\else#2\fi{\fi#1}
\ifx\ifcsname\@undefined\XKV@afterelsefi
  \def\XKV@ifundefined#1{%
    \begingroup\expandafter\expandafter\expandafter\endgroup
      \expandafter\ifx\csname#1\endcsname\relax
      \expandafter\@firstoftwo
    \else
      \expandafter\@secondoftwo
    \fi
  }
\else
  \def\XKV@ifundefined#1{%
    \ifcsname#1\endcsname
      \expandafter\@secondoftwo
    \else
      \expandafter\@firstoftwo
    \fi
  }
\fi
\XKV@ifundefined{ver@keyval.sty}{
  \input keyval
  \expandafter\def\csname ver@keyval.sty\endcsname{1999/03/16}
}{}
\long\def\@ifnextcharacter#1#2#3{%
  \@ifnextchar\bgroup
  {\@ifnextchar{#1}{#2}{#3}}%
  {\@ifncharacter{#1}{#2}{#3}}%
}
\long\def\@ifncharacter#1#2#3#4{%
  \if\string#1\string#4%
    \expandafter\@firstoftwo
  \else
    \expandafter\@secondoftwo
  \fi
  {#2}{#3}#4%
}
\long\def\XKV@for@n#1#2#3{%
  \def#2{#1}%
  \ifx#2\@empty
    \XKV@for@break
  \else
    \expandafter\XKV@f@r
  \fi
  #2{#3}#1,\@nil,%
}
\long\def\XKV@f@r#1#2#3,{%
  \def#1{#3}%
  \ifx#1\@nnil
    \expandafter\@gobbletwo
  \else
    #2\expandafter\XKV@f@r
  \fi
  #1{#2}%
}
\long\def\XKV@for@break #1\@nil,{\fi}
\long\def\XKV@for@o#1{\expandafter\XKV@for@n\expandafter{#1}}
\long\def\XKV@for@en#1#2#3{\XKV@f@r#2{#3}#1,\@nil,}
\long\def\XKV@for@eo#1#2#3{%
  \def#2{\XKV@f@r#2{#3}}\expandafter#2#1,\@nil,%
}
\long\def\XKV@whilist#1#2#3\fi#4{%
  #3\expandafter\XKV@wh@list#1,\@nil,\@nil\@@#2#3\fi{#4}{}\fi
}
\long\def\XKV@wh@list#1,#2\@@#3#4\fi#5#6{%
  \def#3{#1}%
  \ifx#3\@nnil
    \def#3{#6}\expandafter\XKV@wh@l@st
  \else
    #4%
      #5\expandafter\expandafter\expandafter\XKV@wh@list
    \else
      \def#3{#6}\expandafter\expandafter\expandafter\XKV@wh@l@st
    \fi
  \fi
  #2\@@#3#4\fi{#5}{#1}%
}
\long\def\XKV@wh@l@st#1\@@#2#3\fi#4#5{}
\def\XKV@addtomacro@n#1#2{%
  \expandafter\def\expandafter#1\expandafter{#1#2}%
}
\def\XKV@addtomacro@o#1#2{%
  \expandafter\expandafter\expandafter\def
    \expandafter\expandafter\expandafter#1\expandafter
    \expandafter\expandafter{\expandafter#1#2}%
}
\def\XKV@addtolist@n#1#2{%
  \ifx#1\@empty
    \XKV@addtomacro@n#1{#2}%
  \else
    \XKV@addtomacro@n#1{,#2}%
  \fi
}
\def\XKV@addtolist@o#1#2{%
  \ifx#1\@empty
    \XKV@addtomacro@o#1#2%
  \else
    \XKV@addtomacro@o#1{\expandafter,#2}%
  \fi
}
\def\XKV@addtolist@x#1#2{\edef#1{#1\ifx#1\@empty\else,\fi#2}}
\def\@selective@sanitize{\@testopt\@s@lective@sanitize\@M}
\def\@s@lective@sanitize[#1]#2#3{%
  \begingroup
    \count@#1\relax\advance\count@\@ne
    \XKV@toks\expandafter{#3}%
    \def#3{#2}\@onelevel@sanitize#3%
    \edef#3{{#3}{\the\XKV@toks}}%
    \expandafter\@s@l@ctive@sanitize\expandafter#3#3%
  \expandafter\endgroup\expandafter\def\expandafter#3\expandafter{#3}%
}
\def\@s@l@ctive@sanitize#1#2#3{%
  \def\@i{\futurelet\@@tok\@ii}%
  \def\@ii{%
    \expandafter\@iii\meaning\@@tok\relax
    \ifx\@@tok\@s@l@ctive@sanitize
      \let\@@cmd\@gobble
    \else
      \ifx\@@tok\@sptoken
        \XKV@toks\expandafter{#1}\edef#1{\the\XKV@toks\space}%
        \def\@@cmd{\afterassignment\@i\let\@@tok= }%
      \else
        \let\@@cmd\@iv
      \fi
    \fi
    \@@cmd
  }%
  \def\@iii##1##2\relax{\if##1\@backslashchar\let\@@tok\relax\fi}%
  \def\@iv##1{%
    \toks@\expandafter{#1}\XKV@toks{##1}%
    \ifx\@@tok\bgroup
      \advance\count@\m@ne
      \ifnum\count@>\z@
        \begingroup
          \def#1{\expandafter\@s@l@ctive@sanitize
            \csname\string#1\endcsname{#2}}%
          \expandafter#1\expandafter{\the\XKV@toks}%
          \XKV@toks\expandafter\expandafter\expandafter
            {\csname\string#1\endcsname}%
          \edef#1{\noexpand\XKV@toks{\the\XKV@toks}}%
        \expandafter\endgroup#1%
      \fi
      \edef#1{\the\toks@{\the\XKV@toks}}%
      \advance\count@\@ne
      \let\@@cmd\@i
    \else
      \edef#1{\expandafter\string\the\XKV@toks}%
      \expandafter\in@\expandafter{#1}{#2}%
      \edef#1{\the\toks@\ifin@#1\else
              \ifx\@@tok\@sptoken\space\else\the\XKV@toks\fi\fi}%
      \edef\@@cmd{\noexpand\@i\ifx\@@tok\@sptoken\the\XKV@toks\fi}%
    \fi
    \@@cmd
  }%
  \let#1\@empty\@i#3\@s@l@ctive@sanitize
}
\def\XKV@checksanitizea#1#2{%
  \XKV@ch@cksanitize{#1}#2=%
  \ifin@\else\XKV@ch@cksanitize{#1}#2,\fi
  \ifin@\@selective@sanitize[0]{,=}#2\fi
}
\def\XKV@checksanitizeb#1#2{%
  \XKV@ch@cksanitize{#1}#2,%
  \ifin@\@selective@sanitize[0],#2\fi
}
\def\XKV@ch@cksanitize#1#2#3{%
  \def#2{#1}%
  \@onelevel@sanitize#2%
  \@expandtwoargs\in@#3{#2}%
  \ifin@
    \def#2##1#3##2\@nil{%
      \def#2{##2}%
      \ifx#2\@empty\else\in@false\fi
    }%
    #2#1#3\@nil
  \fi
  \def#2{#1}%
}
\def\XKV@sp@deflist#1#2{%
  \let#1\@empty
  \XKV@for@n{#2}\XKV@resa{%
    \expandafter\KV@@sp@def\expandafter\XKV@resa\expandafter{\XKV@resa}%
    \XKV@addtomacro@o#1{\expandafter,\XKV@resa}%
  }%
  \ifx#1\@empty\else
    \def\XKV@resa,##1\@nil{\def#1{##1}}%
    \expandafter\XKV@resa#1\@nil
  \fi
}
\def\XKV@merge#1#2#3{%
  \XKV@checksanitizea{#2}\XKV@tempa
  \XKV@for@o\XKV@tempa\XKV@tempa{%
    \XKV@pltrue
    #3\XKV@tempa\XKV@tempb
    \let\XKV@tempc#1%
    \let#1\@empty
    \XKV@for@o\XKV@tempc\XKV@tempc{%
      #3\XKV@tempc\XKV@tempd
      \ifx\XKV@tempb\XKV@tempd
        \XKV@plfalse
        \XKV@addtolist@o#1\XKV@tempa
      \else
        \XKV@addtolist@o#1\XKV@tempc
      \fi
    }%
    \ifXKV@pl\XKV@addtolist@o#1\XKV@tempa\fi
  }%
  \ifXKV@st\global\let#1#1\fi
}
\def\XKV@delete#1#2#3{%
  \XKV@checksanitizeb{#2}\XKV@tempa
  \let\XKV@tempb#1%
  \let#1\@empty
  \XKV@for@o\XKV@tempb\XKV@tempb{%
    #3\XKV@tempb\XKV@tempc
    \@expandtwoargs\in@{,\XKV@tempc,}{,\XKV@tempa,}%
    \ifin@\else\XKV@addtolist@o#1\XKV@tempb\fi
  }%
  \ifXKV@st\global\let#1#1\fi
}
\def\XKV@warn#1{\message{xkeyval warning: #1}}
\def\XKV@err#1{\errmessage{xkeyval error: #1}}
\def\KV@errx{\XKV@err}
\let\KV@err\KV@errx
\def\XKV@ifstar#1{\@ifnextcharacter*{\@firstoftwo{#1}}}
\def\XKV@ifplus#1{\@ifnextcharacter+{\@firstoftwo{#1}}}
\def\XKV@makepf#1{%
  \KV@@sp@def\XKV@prefix{#1}%
  \def\XKV@resa{XKV}%
  \ifx\XKV@prefix\XKV@resa
    \XKV@err{`XKV' prefix is not allowed}%
    \let\XKV@prefix\@empty
  \else
    \edef\XKV@prefix{\ifx\XKV@prefix\@empty\else\XKV@prefix @\fi}%
  \fi
}
\def\XKV@makehd#1{%
  \expandafter\KV@@sp@def\expandafter\XKV@header\expandafter{#1}%
  \edef\XKV@header{%
    \XKV@prefix\ifx\XKV@header\@empty\else\XKV@header @\fi
  }%
}
\def\XKV@srstate#1#2{%
  \ifx\@empty#2\@empty\advance\XKV@depth\@ne\fi
  \XKV@for@n{XKV@prefix,XKV@fams,XKV@na,ifXKV@st,ifXKV@pl,ifXKV@knf}%
    \XKV@resa{\expandafter\let\csname\XKV@resa#1\expandafter
      \endcsname\csname\XKV@resa#2\endcsname
  }%
  \ifx\@empty#1\@empty\advance\XKV@depth\m@ne\fi
}
\def\XKV@testopta#1{%
  \XKV@ifstar{\XKV@sttrue\XKV@t@stopta{#1}}%
    {\XKV@stfalse\XKV@t@stopta{#1}}%
}
\def\XKV@t@stopta#1{\XKV@ifplus{\XKV@pltrue#1}{\XKV@plfalse#1}}
\def\XKV@testoptb#1{\@testopt{\XKV@t@stoptb#1}{KV}}
\def\XKV@t@stoptb#1[#2]#3{%
  \XKV@makepf{#2}%
  \XKV@makehd{#3}%
  \KV@@sp@def\XKV@tfam{#3}%
  #1%
}
\def\XKV@testoptc#1{\@testopt{\XKV@t@stoptc#1}{KV}}
\def\XKV@t@stoptc#1[#2]#3{%
  \XKV@makepf{#2}%
  \XKV@checksanitizeb{#3}\XKV@fams
  \expandafter\XKV@sp@deflist\expandafter
    \XKV@fams\expandafter{\XKV@fams}%
  \@testopt#1{}%
}
\def\XKV@testoptd#1#2{%
  \XKV@testoptb{%
    \edef\XKV@tempa{#2\XKV@header}%
    \def\XKV@tempb{\@testopt{\XKV@t@stoptd#1}}%
    \expandafter\XKV@tempb\expandafter{\XKV@tempa}%
  }%
}
\def\XKV@t@stoptd#1[#2]#3{%
  \@ifnextchar[{\XKV@sttrue#1{#2}{#3}}{\XKV@stfalse#1{#2}{#3}[]}%
}
\def\XKV@ifcmd#1#2#3{%
  \def\XKV@@ifcmd##1#2##2##3\@nil##4{%
    \def##4{##2}\ifx##4\@nnil
      \def##4{##1}\expandafter\@secondoftwo
    \else
      \expandafter\@firstoftwo
    \fi
  }%
  \XKV@@ifcmd#1#2{\@nil}\@nil#3%
}
\def\XKV@getkeyname#1#2{\expandafter\XKV@g@tkeyname#1=\@nil#2}
\def\XKV@g@tkeyname#1=#2\@nil#3{%
  \XKV@ifcmd{#1}\savevalue#3{\XKV@rkvtrue\XKV@sgfalse}{%
    \XKV@ifcmd{#1}\gsavevalue#3%
      {\XKV@rkvtrue\XKV@sgtrue}{\XKV@rkvfalse\XKV@sgfalse}%
  }%
}
\def\XKV@getsg#1#2{%
  \expandafter\XKV@ifcmd\expandafter{#1}\global#2\XKV@sgtrue\XKV@sgfalse
}
\def\XKV@define@default#1#2{%
  \expandafter\def\csname\XKV@header#1@default\expandafter
    \endcsname\expandafter{\csname\XKV@header#1\endcsname{#2}}%
}
\def\define@key{\XKV@testoptb\XKV@define@key}
\def\XKV@define@key#1{%
  \@ifnextchar[{\XKV@d@fine@k@y{#1}}{%
    \expandafter\def\csname\XKV@header#1\endcsname####1%
  }%
}
\def\XKV@d@fine@k@y#1[#2]{%
  \XKV@define@default{#1}{#2}%
  \expandafter\def\csname\XKV@header#1\endcsname##1%
}
\def\define@cmdkey{\XKV@testoptd\XKV@define@cmdkey{cmd}}
\def\XKV@define@cmdkey#1#2[#3]#4{%
  \ifXKV@st\XKV@define@default{#2}{#3}\fi
  \def\XKV@tempa{\expandafter\def\csname\XKV@header#2\endcsname####1}%
  \begingroup\expandafter\endgroup\expandafter\XKV@tempa\expandafter
    {\expandafter\def\csname#1#2\endcsname{##1}#4}%
}
\def\define@cmdkeys{\XKV@testoptd\XKV@define@cmdkeys{cmd}}
\def\XKV@define@cmdkeys#1#2[#3]{%
  \XKV@sp@deflist\XKV@tempa{#2}%
  \XKV@for@o\XKV@tempa\XKV@tempa{%
    \edef\XKV@tempa{\noexpand\XKV@define@cmdkey{#1}{\XKV@tempa}}%
    \XKV@tempa[#3]{}%
  }%
}
\def\define@choicekey{\XKV@testopta{\XKV@testoptb\XKV@define@choicekey}}
\def\XKV@define@choicekey#1{\@testopt{\XKV@d@fine@choicekey{#1}}{}}
\def\XKV@d@fine@choicekey#1[#2]#3{%
  \toks@{#2}%
  \XKV@sp@deflist\XKV@tempa{#3}\XKV@toks\expandafter{\XKV@tempa}%
  \@ifnextchar[{\XKV@d@fine@ch@icekey{#1}}{\XKV@d@fine@ch@ic@key{#1}}%
}
\def\XKV@d@fine@ch@icekey#1[#2]{%
  \XKV@define@default{#1}{#2}%
  \XKV@d@fine@ch@ic@key{#1}%
}
\def\XKV@d@fine@ch@ic@key#1{%
  \ifXKV@pl\XKV@afterelsefi
    \expandafter\XKV@d@f@ne@ch@ic@k@y
  \else\XKV@afterfi
    \expandafter\XKV@d@f@ne@ch@ic@key
  \fi
  \csname\XKV@header#1\endcsname
}
\def\XKV@d@f@ne@ch@ic@key#1#2{\XKV@d@f@n@@ch@ic@k@y#1{{#2}}}
\def\XKV@d@f@ne@ch@ic@k@y#1#2#3{\XKV@d@f@n@@ch@ic@k@y#1{{#2}{#3}}}
\def\XKV@d@f@n@@ch@ic@k@y#1#2{%
  \edef#1##1{%
    \ifXKV@st\noexpand\XKV@sttrue\else\noexpand\XKV@stfalse\fi
    \ifXKV@pl\noexpand\XKV@pltrue\else\noexpand\XKV@plfalse\fi
    \noexpand\XKV@checkchoice[\the\toks@]{##1}{\the\XKV@toks}%
  }%
  \def\XKV@tempa{\def#1####1}%
  \expandafter\XKV@tempa\expandafter{#1{##1}#2}%
}
\def\define@boolkey{\XKV@t@stopta{\XKV@testoptd\XKV@define@boolkey{}}}
\def\XKV@define@boolkey#1#2[#3]{%
  \ifXKV@pl\XKV@afterelsefi
    \expandafter\XKV@d@f@ne@boolkey
  \else\XKV@afterfi
    \expandafter\XKV@d@fine@boolkey
  \fi
  \csname\XKV@header#2\endcsname{#2}{#1#2}{#3}%
}
\def\XKV@d@fine@boolkey#1#2#3#4#5{%
  \XKV@d@f@ne@b@olkey#1{#2}{#3}{#4}%
    {{\csname#3\XKV@resa\endcsname#5}}%
}
\def\XKV@d@f@ne@boolkey#1#2#3#4#5#6{%
  \XKV@d@f@ne@b@olkey#1{#2}{#3}{#4}%
    {{\csname#3\XKV@resa\endcsname#5}{#6}}%
}
\def\XKV@d@f@ne@b@olkey#1#2#3#4#5{%
  \expandafter\newif\csname if#3\endcsname
  \ifXKV@st\XKV@define@default{#2}{#4}\fi
  \ifXKV@pl
    \def#1##1{\XKV@pltrue\XKV@sttrue
      \XKV@checkchoice[\XKV@resa]{##1}{true,false}#5%
    }%
  \else
    \def#1##1{\XKV@plfalse\XKV@sttrue
      \XKV@checkchoice[\XKV@resa]{##1}{true,false}#5%
    }%
  \fi
}
\def\define@boolkeys{\XKV@plfalse\XKV@testoptd\XKV@define@boolkeys{}}
\def\XKV@define@boolkeys#1#2[#3]{%
  \XKV@sp@deflist\XKV@tempa{#2}%
  \XKV@for@o\XKV@tempa\XKV@tempa{%
    \expandafter\XKV@d@fine@boolkeys\expandafter{\XKV@tempa}{#1}{#3}%
  }%
}
\def\XKV@d@fine@boolkeys#1#2#3{%
  \expandafter\XKV@d@f@ne@b@olkey\csname\XKV@header#1\endcsname
    {#1}{#2#1}{#3}{{\csname#2#1\XKV@resa\endcsname}}%
}
\def\XKV@cc{\XKV@testopta{\@testopt\XKV@checkchoice{}}}
\def\XKV@checkchoice[#1]#2#3{%
  \def\XKV@tempa{#1}%
  \ifXKV@st\lowercase{\fi
  \ifx\XKV@tempa\@empty
    \def\XKV@tempa{\XKV@ch@ckch@ice\@nil{#2}{#3}}%
  \else
    \def\XKV@tempa{\XKV@ch@ckchoice#1\@nil{#2}{#3}}%
  \fi
  \ifXKV@st}\fi\XKV@tempa
}
\def\XKV@ch@ckchoice#1#2\@nil#3#4{%
  \def\XKV@tempa{#2}%
  \ifx\XKV@tempa\@empty\XKV@afterelsefi
    \XKV@ch@ckch@ice#1{#3}{#4}%
  \else\XKV@afterfi
    \XKV@@ch@ckchoice#1#2{#3}{#4}%
  \fi
}
\def\XKV@ch@ckch@ice#1#2#3{%
  \def\XKV@tempa{#1}%
  \ifx\XKV@tempa\@nnil\let\XKV@tempa\@empty\else
    \def\XKV@tempa{\def#1{#2}}%
  \fi
  \in@{,#2,}{,#3,}%
  \ifin@
    \ifXKV@pl
      \XKV@addtomacro@n\XKV@tempa\@firstoftwo
    \else
      \XKV@addtomacro@n\XKV@tempa\@firstofone
    \fi
  \else
    \ifXKV@pl
      \XKV@addtomacro@n\XKV@tempa\@secondoftwo
    \else
      \XKV@toks{#2}%
      \XKV@err{value `\the\XKV@toks' is not allowed}%
      \XKV@addtomacro@n\XKV@tempa\@gobble
    \fi
  \fi
  \XKV@tempa
}
\def\XKV@@ch@ckchoice#1#2#3#4{%
  \edef\XKV@tempa{\the\count@}\count@\z@
  \def\XKV@tempb{#3}%
  \def\XKV@tempc##1,{%
    \def#1{##1}%
    \ifx#1\@nnil
      \def#1{#3}\def#2{-1}\count@\XKV@tempa
      \ifXKV@pl
        \let\XKV@tempd\@secondoftwo
      \else
        \XKV@toks{#3}%
        \XKV@err{value `\the\XKV@toks' is not allowed}%
        \let\XKV@tempd\@gobble
      \fi
    \else
      \ifx#1\XKV@tempb
        \edef#2{\the\count@}\count@\XKV@tempa
        \ifXKV@pl
          \let\XKV@tempd\XKV@@ch@ckch@ice
        \else
          \let\XKV@tempd\XKV@@ch@ckch@ic@
        \fi
      \else
        \advance\count@\@ne
        \let\XKV@tempd\XKV@tempc
      \fi
    \fi
    \XKV@tempd
  }%
  \XKV@tempc#4,\@nil,%
}
\def\XKV@@ch@ckch@ice#1\@nil,{\@firstoftwo}
\def\XKV@@ch@ckch@ic@#1\@nil,{\@firstofone}
\def\key@ifundefined{\@testopt\XKV@key@ifundefined{KV}}
\def\XKV@key@ifundefined[#1]#2{%
  \XKV@makepf{#1}%
  \XKV@checksanitizeb{#2}\XKV@fams
  \expandafter\XKV@sp@deflist\expandafter
    \XKV@fams\expandafter{\XKV@fams}%
  \XKV@key@if@ndefined
}
\def\XKV@key@if@ndefined#1{%
  \XKV@knftrue
  \KV@@sp@def\XKV@tkey{#1}%
  \XKV@whilist\XKV@fams\XKV@tfam\ifXKV@knf\fi{%
    \XKV@makehd\XKV@tfam
    \XKV@ifundefined{\XKV@header\XKV@tkey}{}{\XKV@knffalse}%
  }%
  \ifXKV@knf
    \expandafter\@firstoftwo
  \else
    \expandafter\@secondoftwo
  \fi
}
\def\disable@keys{\XKV@testoptb\XKV@disable@keys}
\def\XKV@disable@keys#1{%
  \XKV@checksanitizeb{#1}\XKV@tempa
  \XKV@for@o\XKV@tempa\XKV@tempa{%
    \XKV@ifundefined{\XKV@header\XKV@tempa}{%
      \XKV@err{key `\XKV@tempa' undefined}%
    }{%
      \edef\XKV@tempb{%
        \noexpand\XKV@warn{key `\XKV@tempa' has been disabled}%
      }%
      \XKV@ifundefined{\XKV@header\XKV@tempa @default}{%
        \edef\XKV@tempc{\noexpand\XKV@define@key{\XKV@tempa}}%
      }{%
        \edef\XKV@tempc{\noexpand\XKV@define@key{\XKV@tempa}[]}%
      }%
      \expandafter\XKV@tempc\expandafter{\XKV@tempb}%
    }%
  }%
}
\def\presetkeys{\XKV@stfalse\XKV@testoptb\XKV@presetkeys}
\def\gpresetkeys{\XKV@sttrue\XKV@testoptb\XKV@presetkeys}
\def\XKV@presetkeys#1#2{%
  \XKV@pr@setkeys{#1}{preseth}%
  \XKV@pr@setkeys{#2}{presett}%
}
\def\XKV@pr@setkeys#1#2{%
  \XKV@ifundefined{XKV@\XKV@header#2}{%
    \XKV@checksanitizea{#1}\XKV@tempa
    \ifXKV@st\expandafter\global\fi\expandafter\def\csname
      XKV@\XKV@header#2\expandafter\endcsname\expandafter{\XKV@tempa}%
  }{%
    \expandafter\XKV@merge\csname XKV@\XKV@header
      #2\endcsname{#1}\XKV@getkeyname
  }%
}
\def\delpresetkeys{\XKV@stfalse\XKV@testoptb\XKV@delpresetkeys}
\def\gdelpresetkeys{\XKV@sttrue\XKV@testoptb\XKV@delpresetkeys}
\def\XKV@delpresetkeys#1#2{%
  \XKV@d@lpresetkeys{#1}{preseth}%
  \XKV@d@lpresetkeys{#2}{presett}%
}
\def\XKV@d@lpresetkeys#1#2{%
  \XKV@ifundefined{XKV@\XKV@header#2}{%
    \XKV@err{no presets defined for `\XKV@header'}%
  }{%
    \expandafter\XKV@delete\csname XKV@\XKV@header
      #2\endcsname{#1}\XKV@getkeyname
  }%
}
\def\unpresetkeys{\XKV@stfalse\XKV@testoptb\XKV@unpresetkeys}
\def\gunpresetkeys{\XKV@sttrue\XKV@testoptb\XKV@unpresetkeys}
\def\XKV@unpresetkeys{%
  \XKV@ifundefined{XKV@\XKV@header preseth}{%
    \XKV@err{no presets defined for `\XKV@header'}%
  }{%
    \ifXKV@st\expandafter\global\fi\expandafter\let
      \csname XKV@\XKV@header preseth\endcsname\@undefined
    \ifXKV@st\expandafter\global\fi\expandafter\let
      \csname XKV@\XKV@header presett\endcsname\@undefined
  }%
}
\def\savekeys{\XKV@stfalse\XKV@testoptb\XKV@savekeys}
\def\gsavekeys{\XKV@sttrue\XKV@testoptb\XKV@savekeys}
\def\XKV@savekeys#1{%
  \XKV@ifundefined{XKV@\XKV@header save}{%
    \XKV@checksanitizeb{#1}\XKV@tempa
    \ifXKV@st\expandafter\global\fi\expandafter\def\csname XKV@%
      \XKV@header save\expandafter\endcsname\expandafter{\XKV@tempa}%
  }{%
    \expandafter\XKV@merge\csname XKV@\XKV@header
      save\endcsname{#1}\XKV@getsg
  }%
}
\def\delsavekeys{\XKV@stfalse\XKV@testoptb\XKV@delsavekeys}
\def\gdelsavekeys{\XKV@sttrue\XKV@testoptb\XKV@delsavekeys}
\def\XKV@delsavekeys#1{%
  \XKV@ifundefined{XKV@\XKV@header save}{%
    \XKV@err{no save keys defined for `\XKV@header'}%
  }{%
    \expandafter\XKV@delete\csname XKV@\XKV@header
      save\endcsname{#1}\XKV@getsg
  }%
}
\def\unsavekeys{\XKV@stfalse\XKV@testoptb\XKV@unsavekeys}
\def\gunsavekeys{\XKV@sttrue\XKV@testoptb\XKV@unsavekeys}
\def\XKV@unsavekeys{%
  \XKV@ifundefined{XKV@\XKV@header save}{%
    \XKV@err{no save keys defined for `\XKV@header'}%
  }{%
    \ifXKV@st\expandafter\global\fi\expandafter\let
      \csname XKV@\XKV@header save\endcsname\@undefined
  }%
}
\def\setkeys{\XKV@testopta{\XKV@testoptc\XKV@setkeys}}
\def\XKV@setkeys[#1]#2{%
  \XKV@checksanitizea{#2}\XKV@resb
  \let\XKV@naa\@empty
  \XKV@for@o\XKV@resb\XKV@tempa{%
    \expandafter\XKV@g@tkeyname\XKV@tempa=\@nil\XKV@tempa
    \XKV@addtolist@x\XKV@naa\XKV@tempa
  }%
  \let\XKV@rm\@empty
  \XKV@usepresetkeys{#1}{preseth}%
  \expandafter\XKV@s@tkeys\expandafter{\XKV@resb}{#1}%
  \XKV@usepresetkeys{#1}{presett}%
}
\def\XKV@usepresetkeys#1#2{%
  \XKV@presettrue
  \XKV@for@eo\XKV@fams\XKV@tfam{%
    \XKV@makehd\XKV@tfam
    \XKV@ifundefined{XKV@\XKV@header#2}{}{%
      \XKV@toks\expandafter\expandafter\expandafter
        {\csname XKV@\XKV@header#2\endcsname}%
      \@expandtwoargs\XKV@s@tkeys{\the\XKV@toks}%
        {\XKV@naa\ifx\XKV@naa\@empty\else,\fi#1}%
    }%
  }%
  \XKV@presetfalse
}
\def\XKV@s@tkeys#1#2{%
  \XKV@sp@deflist\XKV@na{#2}%
  \XKV@for@n{#1}\CurrentOption{%
    \expandafter\XKV@s@tk@ys\CurrentOption==\@nil
  }%
}
\def\XKV@s@tk@ys#1=#2=#3\@nil{%
  \XKV@g@tkeyname#1=\@nil\XKV@tkey
  \expandafter\KV@@sp@def\expandafter\XKV@tkey\expandafter{\XKV@tkey}%
  \ifx\XKV@tkey\@empty
    \XKV@toks{#2}%
    \ifcat$\the\XKV@toks$\else
      \XKV@err{no key specified for value `\the\XKV@toks'}%
    \fi
  \else
    \@expandtwoargs\in@{,\XKV@tkey,}{,\XKV@na,}%
    \ifin@\else
      \XKV@knftrue
      \KV@@sp@def\XKV@tempa{#2}%
      \ifXKV@preset\XKV@s@tk@ys@{#3}\else
        \ifXKV@pl
          \XKV@for@eo\XKV@fams\XKV@tfam{%
            \XKV@makehd\XKV@tfam
            \XKV@s@tk@ys@{#3}%
          }%
        \else
          \XKV@whilist\XKV@fams\XKV@tfam\ifXKV@knf\fi{%
            \XKV@makehd\XKV@tfam
            \XKV@s@tk@ys@{#3}%
          }%
        \fi
      \fi
      \ifXKV@knf
        \ifXKV@inpox
          \ifx\XKV@doxs\relax
            \ifx\@currext\@clsextension\else
              \let\CurrentOption\XKV@tkey\@unknownoptionerror
            \fi
          \else\XKV@doxs\fi
        \else
          \ifXKV@st
            \global\XKV@addtolist@o\XKV@rm\CurrentOption
          \else
            \XKV@err{`\XKV@tkey' undefined in families `\XKV@fams'}%
          \fi
        \fi
      \else
        \ifXKV@inpox\ifx\XKV@testclass\XKV@documentclass
          \expandafter\XKV@useoption\expandafter{\CurrentOption}%
        \fi\fi
      \fi
    \fi
  \fi
}
\def\XKV@s@tk@ys@#1{%
  \XKV@ifundefined{\XKV@header\XKV@tkey}{}{%
    \XKV@knffalse
    \XKV@ifundefined{XKV@\XKV@header save}{}{%
      \expandafter\XKV@testsavekey\csname XKV@\XKV@header
        save\endcsname\XKV@tkey
    }%
    \ifXKV@rkv
      \ifXKV@sg\expandafter\global\fi\expandafter\let
        \csname XKV@\XKV@header\XKV@tkey @value\endcsname\XKV@tempa
    \fi
    \expandafter\XKV@replacepointers\expandafter{\XKV@tempa}%
    \ifx\@empty#1\@empty\XKV@afterelsefi
      \XKV@ifundefined{\XKV@header\XKV@tkey @default}{%
        \XKV@err{no value specified for key `\XKV@tkey'}%
      }{%
        \expandafter\expandafter\expandafter\XKV@default
          \csname\XKV@header\XKV@tkey @default\endcsname\@nil
      }%
    \else\XKV@afterfi
      \XKV@srstate{@\romannumeral\XKV@depth}{}%
      \csname\XKV@header\XKV@tkey\expandafter
        \endcsname\expandafter{\XKV@tempa}\relax
      \XKV@srstate{}{@\romannumeral\XKV@depth}%
    \fi
  }%
}
\def\XKV@testsavekey#1#2{%
  \ifXKV@rkv\else
    \XKV@for@o#1\XKV@resa{%
      \expandafter\XKV@ifcmd\expandafter{\XKV@resa}\global\XKV@resa{%
        \ifx#2\XKV@resa
          \XKV@rkvtrue\XKV@sgtrue
        \fi
      }{%
        \ifx#2\XKV@resa
          \XKV@rkvtrue\XKV@sgfalse
        \fi
      }%
    }%
  \fi
}
\def\XKV@replacepointers#1{%
  \let\XKV@tempa\@empty
  \let\XKV@resa\@empty
  \XKV@r@placepointers#1\usevalue\@nil
}
\def\XKV@r@placepointers#1\usevalue#2{%
  \XKV@addtomacro@n\XKV@tempa{#1}%
  \def\XKV@tempb{#2}%
  \ifx\XKV@tempb\@nnil\else\XKV@afterfi
    \XKV@ifundefined{XKV@\XKV@header#2@value}{%
      \XKV@err{no value recorded for key `#2'; ignored}%
      \XKV@r@placepointers
    }{%
      \@expandtwoargs\in@{,#2,}{,\XKV@resa,}%
      \ifin@\XKV@afterelsefi
        \XKV@err{back linking pointers; pointer replacement canceled}%
      \else\XKV@afterfi
        \XKV@addtolist@x\XKV@resa{#2}%
        \expandafter\expandafter\expandafter\XKV@r@placepointers
          \csname XKV@\XKV@header#2@value\endcsname
      \fi
    }%
  \fi
}
\def\XKV@default#1#2\@nil{%
  \expandafter\edef\expandafter\XKV@tempa
    \expandafter{\expandafter\@gobble\string#1}%
  \edef\XKV@tempb{\XKV@header\XKV@tkey}%
  \@onelevel@sanitize\XKV@tempb
  \ifx\XKV@tempa\XKV@tempb
    \begingroup
      \expandafter\def\csname\XKV@header\XKV@tkey\endcsname##1{%
        \gdef\XKV@tempa{##1}%
      }%
      \csname\XKV@header\XKV@tkey @default\endcsname
    \endgroup
    \XKV@ifundefined{XKV@\XKV@header save}{}{%
      \expandafter\XKV@testsavekey\csname XKV@\XKV@header
        save\endcsname\XKV@tkey
    }%
    \ifXKV@rkv
      \ifXKV@sg\expandafter\global\fi\expandafter\let
        \csname XKV@\XKV@header\XKV@tkey @value\endcsname\XKV@tempa
    \fi
    \expandafter\XKV@replacepointers\expandafter
      {\XKV@tempa}\XKV@afterelsefi
    \XKV@srstate{@\romannumeral\XKV@depth}{}%
    \expandafter#1\expandafter{\XKV@tempa}\relax
    \XKV@srstate{}{@\romannumeral\XKV@depth}%
  \else\XKV@afterfi
    \XKV@srstate{@\romannumeral\XKV@depth}{}%
    \csname\XKV@header\XKV@tkey @default\endcsname\relax
    \XKV@srstate{}{@\romannumeral\XKV@depth}%
  \fi
}
\def\setrmkeys{\XKV@testopta{\XKV@testoptc\XKV@setrmkeys}}
\def\XKV@setrmkeys[#1]{%
  \def\XKV@tempa{\XKV@setkeys[#1]}%
  \expandafter\XKV@tempa\expandafter{\XKV@rm}%
}
\XKVcatcodes
\endinput
%%
%% End of file `xkeyval.tex'.


==> xypdf-c.tex <==
%auto-ignore
%this ensures the arxiv doesn't try to start TeXing here.
%% xypdf-c.tex from $Id: xypdf-c.doc,v $
%%
%% Xy-pic ``Colour extension'' PDF backend support.
%% Copyright (c) 1999-1999 Ross Moore <ross@mpce.mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-1999 Kristoffer H. Rose <krisrose@brics.dk>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, write to the Free Software Foundation, Inc.,
%% 675 Mass Ave, Cambridge, MA 02139, USA.
%%
%% As a special exception, you may use this file and all files derived
%% from it without restrictions. This special exception was added with
%% version 3.7 of Xy-pic.
%%
\expandafter\ifx\csname xypdf-cloaded\endcsname\empty
 \message{not reloaded}\endinput \fi
\expandafter\let\csname xypdf-cloaded\endcsname=\empty \xycatcodes
\expandafter\ifx \csname xypdf-sloaded\endcsname\empty\else
 \xyinputorelse@{xypdf-s}{\xyerror@{Could not load xypdf-s}{}}%
 \xycatcodes\fi
\xydef@\UsePDFcolor{\installPDFcolor@}
\xydef@\NoPDFcolor{\UnloadColor@}
\xydef@\installPDFcolor@{\installPDFstyle@
 \let\xymath@=\xyPDFmath@ \let\xynomath@=\xyPDFnomath@
 \let\checkxyPDFcolor@=\checkxyPDFcolor@@
 \let\xycolor@@=\xyPDFcolor@@
 \xystandardcolors@
 \xyuncatcodes }
\xydef@\xyPDFmath@{\hbox\bgroup\dimen@=.55ex \checkxyPDFcolor@ \xyinside@}
\xydef@\xyPDFnomath@{\hbox\bgroup\dimen@=\z@ \checkxyPDFcolor@ \xyinside@}
\xydef@\checkxyPDFcolor@@{\edef\pdfsaved@color{\pdfcurrent@color}%
 \let\checkxyPDFcolor@=\relax}
\xylet@\checkxyPDFcolor@=\relax
\xydef@\xyPDFnewcolor@#1#2#3#4#5{%
 \expandafter\DN@\expandafter{\csname shape [#1]\endcsname}%
 \DNii@{\relax}\ifx\next@\nextii@\newxycolor{#1}{}\relax\fi
 \DNii@{#4}\ifx\nextii@\empty
 \expandafter\DNii@\expandafter{\csname xyPDFshape@#1@\endcsname}%
 \expandafter\def\nextii@{\xyPDFcolor@{#2//#3}}\else
 \expandafter\DNii@\expandafter{\csname xyPDFshape@#1@\endcsname}%
 \expandafter\def\nextii@{\xyPDFcolor@{#4}}\fi
 \ifx\nextii@\empty\expandafter\def\next@{\xyPDFnotimplemented@@`#1'@@}%
 \else
 \edef\tmp@{\noexpand\let\expandafter\noexpand\next@
 \expandafter\noexpand\nextii@}\expandafter\tmp@\fi }
\xylet@\newxycolor@=\xyPDFnewcolor@
\xydef@\xyPDFcolor@{\ifPDFspecials@\expandafter\xyPDFcolor@@
 \else\expandafter\eat@\fi}
\xydef@\xyPDFcolor@@#1{\bgroup \checkXyStyle@
 \def\preStyle@@{\expandafter\addtostyletoks@\expandafter{\xyPDFpre@}}%
 \def\postStyle@@{\expandafter\addtostyletoks@\expandafter{\xyPDFpost@}}%
 \let\modPDFboxz@=\modXYstyle@ \xyPDF@color@@{#1}%
 \toks@={\egroup\let\xy@style@=\relax \def\Drop@@}%
 \expandafter\addtotoks@\expandafter{\expandafter{\Drop@@}\def\Connect@@}%
 \expandafter\addtotoks@\expandafter{\expandafter{\Connect@@}}%
 \the\toks@ }

\xydef@\pdfcurrent@color{1 1 1 1 k 1 1 1 1 K}
\xydef@\pdfsaved@color{1 1 1 1 k 1 1 1 1 K}
\xydef@\xyPDF@color@@#1{%
 \edef\pdfsaved@color{\pdfcurrent@color}%
 \pdf@convertcolor#1////!%
 \edef\next@{\noexpand\xyPDFsplitPDF@{\pdfcurrent@color}{\pdfsaved@color}}%
 \next@}
\xydef@\pdf@convertcolor#1//#2//#3!{\DN@{#2}%
 \DNii@{cmyk}\ifx\next@\nextii@\DN@{#1 k #1 K}%
 \else \DNii@{rgb}\ifx\next@\nextii@\DN@{#1 rg #1 RG}%
 \else \DNii@{gray}\ifx\next@\nextii@\DN@{#1 #1 #1 rg #1 #1 #1 RG}%
 \else \DN@{1 1 1 1 k 1 1 1 1 K}%
 \fi \fi \fi
 \expandafter\def\expandafter\pdfcurrent@color\expandafter{\next@}}
\xydef@\xycolor@raw@@#1{}%
\endinput


==> xypdf-f.tex <==
%auto-ignore
%this ensures the arxiv doesn't try to start TeXing here.
%% xypdf-f.tex from $Id: xypdf-f.doc,v $
%%
%% Xy-pic ``Frame extension'' PDF backend support.
%% Copyright (c) 1999-1999 Ross Moore <ross@mpce.mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-1999 Kristoffer H. Rose <krisrose@brics.dk>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, write to the Free Software Foundation, Inc.,
%% 675 Mass Ave, Cambridge, MA 02139, USA.
%%
%% As a special exception, you may use this file and all files derived
%% from it without restrictions. This special exception was added with
%% version 3.7 of Xy-pic.
%%
\expandafter\ifx\csname xypdf-floaded\endcsname\empty
 \message{not reloaded}\endinput \fi
\expandafter\let\csname xypdf-floaded\endcsname=\empty \xycatcodes
\xydef@\installPDFframes@{%
 \let\framed@body@@=\xyPDFframed@body@
 \let\circled@x@@=\xyPDFcircled@x@
 \let\ellipsed@x@@=\xyPDFellipsed@x@
 \installPDFfills@
 \xyuncatcodes}
\xydef@\UsePDFframes{\installPDFframes@}
\xydef@\NoPDFframes{\UnloadFrames@}
\xydef@\xyPDFframed@body@{\DN@{\framed@body@}%
 \ifx\framehfill\frm@solidh@@
 \DN@{\xyPDFframed@oval@\xyPDFoval@Special}%
 \else\ifdim\R@=\z@\else
 \ifx\framehfill\frm@dashh@@
 \DN@{\xyPDFframed@oval@\xyPDFdashoval@Special}%
 \else\ifx\framehfill\frm@doth@@
 \DN@{\xyPDFframed@oval@\xyPDFdotoval@Special}%
 \fi\fi
 \fi\fi \next@ }
\xydef@\xyPDFframed@oval@#1{\vglue\U@c
 \hbox{\hglue\L@c\xypdfoval@#1\hglue\R@c}\vglue\D@c}
\xydef@\xyPDFcircled@x@{\DN@{\xyPDFcircled@x@@\xyPDFcirc@Special}%
 \ifx\framehfill\frm@doth@@
 \DN@{\xyPDFcircled@x@@\xyPDFdotcirc@Special}%
 \else\ifx\framehfill\frm@dashh@@
 \DN@{\xyPDFcircled@x@@\xyPDFdashcirc@Special}%
 \fi\fi \next@ }
\xydef@\xyPDFcircled@x@@#1{\vglue2\R@
 \hbox{\hglue2\R@\xypdfcircle@#1\hglue2\R@}%
 \vglue2\R@}
\xydef@\xyPDFellipsed@x@#1#2{%
 \DN@{\xyPDFellipsed@x@@\xyPDFcirc@Special}%
 \ifx\framehfill\frm@doth@@
 \DN@{\xyPDFellipsed@x@@\xyPDFdotcirc@Special}%
 \else\ifx\framehfill\frm@dashh@@
 \DN@{\xyPDFellipsed@x@@\xyPDFdashcirc@Special}%
 \fi\fi \next@{#1}{#2}}
\xydef@\xyPDFellipsed@x@@#1#2#3{\vglue #3\vglue #3\relax
 \hbox{\L@c = #2\relax \R@c=\L@c \D@c = #3\relax \U@c=\D@c
 \hglue#2\hglue#2\relax\xypdfellipse@#1\hglue#2\hglue#2\relax}%
 \vglue #3\vglue #3\relax}
\xydef@\xyPDFdashhfill@{{\SemiDirectionChar=95 \Direction=3072 \xyPDFdash@}}
\xydef@\xyPDFdashvfill@{{\SemiDirection=31 \Direction=1023 \xyPDFdash@}}
\xydef@\xypdfoval@#1{%
 \dimen@=\L@c \advance\dimen@\R@c
 \dimen@ii=\U@c \advance\dimen@ii\D@c
 \ifdim\dimen@ii<\dimen@ \relax \dimen@=\dimen@ii\fi \divide\dimen@\tw@
 \ifdim\R@>\dimen@ \relax \R@=\dimen@ \fi
 \D@c=-\D@c \L@c=-\L@c
 \edef\tmp@{\expandafter\removePT@\the\R@
 \space\expandafter\removePT@\the\R@c
 \space\expandafter\removePT@\the\D@c
 \space\expandafter\removePT@\the\L@c
 \space\expandafter\removePT@\the\U@c }%
 \expandafter#1\expandafter{\tmp@}}
\xydef@\xypdfcircle@#1{\dimen@=\R@
 \edef\tmp@{\expandafter\removePT@\the\dimen@}%
 \expandafter#1\expandafter{\tmp@}}
\xydef@\xypdfellipse@#1{\edef\tmp@{%
 \expandafter\removePT@\the\U@c \space
 \expandafter\removePT@\the\D@c \space
 \expandafter\removePT@\the\L@c \space
 \expandafter\removePT@\the\R@c }%
 \expandafter#1\expandafter{\tmp@}}
\xydef@\xyPDFoval@Special#1{\PDFmacro@{#1 ov}}%%%%<<<---- here
\xydef@\xyPDFcirc@Special#1{\PDFmacro@{#1 ox}}%%%%<<<---- here
\xydef@\xyPDFdotcirc@Special#1{\PDFmacro@{#1 ot}}%%%%<<<---- here
\xydef@\xyPDFdashcirc@Special#1{\PDFmacro@{#1 od}}%%%%<<<---- here
\xydef@\xyPDFdotoval@Special#1{\PDFmacro@{#1 vt}}%%%%<<<---- here
\xydef@\xyPDFdashoval@Special#1{\PDFmacro@{#1 vd}}%%%%<<<---- here
\xydef@\xyPDFfilledRegion#1#2{\setboxz@h{\lower\D@c\vbox{%
 \vglue\U@c\hbox{#1#2\empty\hglue\L@c\hglue\R@c}\vglue\D@c}}%
 \ht\z@=\z@ \dp\z@=\z@ \wd\z@=\z@ \boxz@}
\xydef@\filledRectangle@PDF{%
 \xyPDFfilledRegion{\xypdfoval@\xyPDFfilloval@Special}}
\xydef@\filledCircle@PDF#1{{\R@c=\R@ \L@c=\R@ \U@c=\R@ \D@c=\R@
 \xyPDFfilledRegion{\xypdfcircle@\xyPDFfillcirc@Special}#1}}
\xydef@\filledEllipse@PDF{%
 \xyPDFfilledRegion{\xypdfellipse@\xyPDFfillellipse@Special}}
\xydef@\filledOval@PDF{%
 \xyPDFfilledRegion{\xypdfoval@\xyPDFfilloval@Special}}
\xydef@\frame@emph@PDF#1{\filled@{#1}\relax}
\xydef@\installPDFfills@{%
 \let\frame@emph@@=\frame@emph@PDF
 \let\filledRectangle@@=\filledRectangle@PDF
 \let\filledOval@@=\filledOval@PDF
 \let\filledCircle@@=\filledCircle@PDF
 \let\filledEllipse@@=\filledEllipse@PDF
}
\xydef@\xyPDFfilloval@Special#1#2{%
 \ifx#2\relax\PDFmacro@{#1 sfo}%%%%%<<<---- here
 \else\PDFmacro@{#1 fo}\fi}%%%%<<<---- here
\xydef@\xyPDFfillcirc@Special#1#2{%
 \ifx#2\relax\PDFmacro@{#1 sfc}%%%%%<<<---- here
 \else\PDFmacro@{#1 fc}\fi}%%%%<<<---- here
\xydef@\xyPDFfillellipse@Special#1#2{%
 \ifx#2\relax\PDFmacro@{#1 sfe}%%%%%<<<---- here
 \else\PDFmacro@{#1 fe}\fi}%%%%<<<---- here
\endinput


==> xypdf-l.tex <==
%auto-ignore
%this ensures the arxiv doesn't try to start TeXing here.
%% xypdf-l.tex from $Id: xypdf-l.doc,v $
%%
%% Xy-pic ``Line extension'' PDF backend support.
%% Copyright (c) 1999-1999 Ross Moore <ross@mpce.mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-1999 Kristoffer H. Rose <krisrose@brics.dk>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, write to the Free Software Foundation, Inc.,
%% 675 Mass Ave, Cambridge, MA 02139, USA.
%%
%% As a special exception, you may use this file and all files derived
%% from it without restrictions. This special exception was added with
%% version 3.7 of Xy-pic.
%%
\expandafter\ifx\csname xypdf-lloaded\endcsname\empty
 \message{not reloaded}\endinput \fi
\expandafter\let\csname xypdf-lloaded\endcsname=\empty \xycatcodes
\expandafter\ifx\csname xypdf-sloaded\endcsname\empty\else
 \xyinputorelse@{xypdf-s}{\xyerror@{Could not load xypdf-s}{}}%
 \xycatcodes\fi
\xydef@\installPDFline@{\installPDFstyle@
 \installPDFlinestyles@ \installPDFpolylines@ }
\xydef@\UsePDFlines{\installPDFline@}
\xydef@\NoPDFlines{\UnloadLine@\relax}
\xydef@\xyPDFlineSpecial@#1{\xyPDFrawZ@{ #1 w}}
\xydef@\xyPDFcapSpecial@#1{\xyPDFrawZ@{ #1 J}}
\xydef@\xyPDFjoinSpecial@#1{\xyPDFrawZ@{ #1 j}}
\xydef@\xyPDFmiterSpecial@#1{\xyPDFrawZ@{ #1 M}}
\xydef@\installPDFlinestyles@{%
 \let\xylinewidth@@=\xylinewidth@
 \let\transxyline@@=\transxyline@
 \let\xylineSpecial@@=\xyPDFlineSpecial@
 \let\resetxyline@@=\resetxyline@i
 \let\xy@linecap@@=\xy@linecap@
 \let\xycapSpecial@@=\xyPDFcapSpecial@
 \let\resetxylinecap@@=\resetxylinecap@i
 \let\xy@linejoin@@=\xy@linejoin@
 \let\xyjoinSpecial@@=\xyPDFjoinSpecial@
 \let\resetxylinejoin@@=\resetxylinejoin@i
 \let\xy@linemiter@@=\xy@linemiter@
 \let\xymiterSpecial@@=\xyPDFmiterSpecial@
 \let\resetxylinemiter@@=\resetxylinemiter@i
}
\xydef@\xypolylinePDF@Special#1{\PDFspecial@@{ q [] 0 d #1 S Q}}
\xydef@\xypolydotPDF@Special#1{\PDFspecial@@{ q [1 3] 0 d S Q}}
\xydef@\xypolydashPDF@Special#1{\PDFspecial@@{ q [5] 0 d #1 S Q}}
\xydef@\xypolyfillPDF@Special#1{\PDFspecial@@{ q #1 f Q}}
\xydef@\xypolyeofillPDF@Special#1{\PDFmacro@{ q #1 f* Q}}
\xydef@\installPDFpolylines@{%
 \let\xypolyline@Special=\xypolylinePDF@Special
 \let\xypolydot@Special=\xypolydotPDF@Special
 \let\xypolydash@Special=\xypolydashPDF@Special
 \let\xypolyfill@Special=\xypolyfillPDF@Special
%\let\xypolyeofill@Special=\xypolyeofillPDF@Special
 \let\xy@polystyle@@=\xy@polystyle@ }
\endinput


==> xypdf-r.tex <==
%auto-ignore
%this ensures the arxiv doesn't try to start TeXing here.
%% xypdf-r.tex from $Id: xypdf-r.doc,v $
%%
%% Xy-pic ``PDF Rotations and Scaling''.
%% Copyright (c) 1999-1999 Ross Moore <ross@maths.mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-1999 Kristoffer H. Rose <krisrose@brics.dk>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, write to the Free Software Foundation, Inc.,
%% 675 Mass Ave, Cambridge, MA 02139, USA.
%%
%% As a special exception, you may use this file and all files derived
%% from it without restrictions. This special exception was added with
%% version 3.7 of Xy-pic.
%%
\expandafter\ifx\csname xypdf-rloaded\endcsname\empty
 \message{not reloaded}\endinput \fi
\expandafter\let\csname xypdf-rloaded\endcsname=\empty \xycatcodes
\expandafter\ifx\csname xypdf-sloaded\endcsname\empty\else
 \xyinputorelse@{xypdf-s}{\xyerror@{Could not load xypdf-s}{}}%
 \xycatcodes\fi
\xydef@\installPDFrotscale@{\installPDFstyle@
% \let\xyRotate@@=\xyPDFrotate@@
% \let\doSpecialRotate@@=\doPDFspecialRotate@@
 \let\xyscale@@=\xyPDFscale@@
 \xyPDFshapes@true
 \xyuncatcodes }
\xydef@\UsePDFrotate{\installPDFrotscale@}
\xydef@\NoPDFrotate{\UnloadRotate@\relax}
\xydef@\xyPDFpretransform@{\xyPDFrawA@{\preXYtransform@@}}
\xydef@\xyPDFposttransform@{\xyPDFrawZ@{\postXYtransform@@}}
\let\preXYtransform@=\xyPDFpretransform@
\let\postXYtransform@=\xyPDFposttransform@
\xydef@\xyPDFrotSplit@{%
 \expandafter\def\expandafter\preShape@@\expandafter{\xyPDFpre@}%
 \expandafter\def\expandafter\postShape@@\expandafter{\xyPDFpost@}}
\xydef@\xyPDFscale@@#1#2{%
 \xyPDFsplitPDF@{\xyscale@start(#1,#2)}{\xyscale@end}%
 \xyPDFrotSplit@\xyPDFpdfxy@ }
\xydef@\xyPDFrotate@@#1{%
 \xyPDFsplitPDF@{\xyrot@start(#1 xyd)}{\xyrot@end}%%%<<------ here
 \xyPDFrotSplit@\xyPDFpdfxy@ }
\xydef@\xyPDFspecialRotate@#1{%
 \xyPDFsplitPDF@{\xyrot@start(#1)}{\xyrot@end}\xyPDFrotSplit@\xyPDFpdfxy@ }
\xydef@\doPDFspecialRotate@@#1@@{\xyPDFspecialRotate@{#1}}
\xydef@\xyRotScale@@{%
% \def\xyrot@start(##1){{xyt ##1\space xyr}}%%%<<------ here
 \def\xyscale@start(##1,##2){ q ##1 0 0 ##2 0 0 cm}%
 \def\xyrot@end{ Q}\def\xyscale@end{ Q}}
\endinput


==> xypdf-s.tex <==
%auto-ignore
%this ensures the arxiv doesn't try to start TeXing here.
%% xypdf-s.tex from $Id: xypdf-s.doc,v $
%%
%% Xy-pic ``Style extension'' PDF support.
%% Copyright (c) 1999-1999 Ross Moore <ross@mpce.mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-1999 Kristoffer H. Rose <krisrose@brics.dk>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, write to the Free Software Foundation, Inc.,
%% 675 Mass Ave, Cambridge, MA 02139, USA.
%%
%% As a special exception, you may use this file and all files derived
%% from it without restrictions. This special exception was added with
%% version 3.7 of Xy-pic.
%%
\expandafter\ifx\csname xypdf-sloaded\endcsname\empty
 \message{not reloaded}\endinput \fi
\expandafter\let\csname xypdf-sloaded\endcsname=\empty \xycatcodes
\xydef@\xykillstyles@@{\Unloadstyle@}%
\xywarnifdefined\xyPDFescapestyle@
\xywarnifdefined\xyPDFsplitescape@
{\xyuncatcodes \catcode`@=11
 \gdef\xyPDFescapestyle@#1@@{\xyPDFsplitescape@#1<><>@@}%
 \gdef\xyPDFsplitescape@#1<>#2<>#3@@{\xyescape@@{#1}{#2}}}
\xydef@\xyPDFsplitPDF@#1#2{%
 \def\xyPDFpre@{#1}\def\xyPDFpost@{#2}\modPDFboxz@ }
\xydef@\xyescape@@#1#2{\checkXyStyle@
 \applyFIFOstyle@\prexyescape@{#1}\postxyescape@{#2}}
\xydef@\prexyescape@{\xyescapeSpecial@}
\xydef@\postxyescape@{\xyescapeSpecial@}
\xylet@\xyescapeSpecial@=\eat@
\let\xyescapeSpecial@=\addtostyletoks@
\xydef@\installPDFstyle@{%
 \def\preXYstyle@@{\xyPDFpre@}%
 \let\xydoprestyles@=\xyPDFrawstyleA@
 \let\xydopoststyles@=\xyPDFrawZ@
 \let\xykillstyles@=\xykillstyles@@
 }
\xydef@\xyPDFrawstyleA@#1{\xyPDFrawA@{{#1}{}}}
\endinput


==> xypdfpdf.tex <==
%auto-ignore
%this ensures the arxiv doesn't try to start TeXing here.
%% xypdfpdf.tex from $Id: xypdfpdf.doc,v $
%%
%% Xy-pic ``PDF-PDF'' PDF support.
%% Copyright (c) 1999-1999 Ross Moore <ross@mpce.mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-1999 Kristoffer H. Rose <krisrose@ens-lyon.fr>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, write to the Free Software Foundation, Inc.,
%% 675 Mass Ave, Cambridge, MA 02139, USA.
%%
%% As a special exception, you may use this file and all files derived
%% from it without restrictions. This special exception was added with
%% version 3.7 of Xy-pic.
%%
\expandafter\ifx\csname xypdf-pdfloaded\endcsname\empty
 \message{not reloaded}\endinput \fi
\expandafter\let\csname xypdf-pdfloaded\endcsname=\empty \xycatcodes
\global\newif\ifPDFspecials@
\xylet@\PDFmacro@@=\eat@
\xylet@\PDFdict@@=\eat@
\xylet@\PDFspecial@@=\eat@
\xylet@\PDFread@@=\eat@
\xylet@\PDFinclude@@=\eat@
\xylet@\PDFraw@@=\eat@
\xylet@\xyPDFobeylines@@=\relax
\xylet@\PDFspecialdict@@=\eat@
\xydef@\UnloadPDFpdf@{%
 \let\PDFmacro@@=\eat@
 \let\PDFdict@@=\eat@
 \let\PDFspecial@@=\eat@
 \let\PDFread@@=\eat@
 \let\PDFinclude@@=\eat@
 \let\PDFraw@@=\eat@
 \let\xyPDFobeylines@@=\relax
 \let\PDFspecialdict@@=\eat@
}
\xydef@\UnloadPDF@{\UnloadPDFpdf@
 \expandafter\ifx\csname xypdfloaded\endcsname\unknown\PDFspecials@false
 \else\expandafter\NoPDFspecials\fi}
\xylet@\UnloadPDF@@=\UnloadPDF@
\ifx\undefined\dvitype@\xydef@\dvitype@{null}\fi
\xylet@\xyrealshipout@=\shipout
\xydef@\xyPDFshipout@{\xyrealshipout@}
\xydef@\firstPDF@{%
 \global\let\firstPDF@@=\relax \global\let\firstPDF@=\relax}
\xylet@\firstPDF@@=\firstPDF@
\xylet@\dumpPDFdict@@=\relax
\xydef@\installxypdf@{%
 \xyinputorelse@{xypdfpdf}{\xydrivernoload@{pdfpdf}}\xycatcodes
 \installxypdf@@ \installxypdf@x }
\xylet@\installxypdf@@=\relax
\xylet@\setupxyPDF@@=\PDFspecials@true
\xywithoption{pdf}{\let\setupxyPDF@@=\setupxyPDF@}
\xydef@\installxypdf@x{
 \let\firstPDF@=\relax
 \let\XYpredict@=\relax
 \setupxyPDF@@ }
\xydef@\setupxyPDF@{\PDFspecials@true}
\let\realinstallxypdf@x=\installxypdf@x
\ifx\undefined\AfterBeginDocument
 \def\installxypdf@x{\xysetup@@{\realinstallxypdf@x}}%
\else
 \def\installxypdf@x{\AfterBeginDocument{\realinstallxypdf@x}}%
\fi
\xydef@\xydefaultdriver@{dvipdf}
\xydef@\xyPDFdriver#1{\def\xydefaultdriver@{#1}}
\xydef@\installxypdf@orig{\DN@{}%
 \ifx\xydriversselected@@\empty
 \DN@{\expandafter\defaultinstallpdf@\expandafter{\xydefaultdriver@}}%
 \else \def\do##1{%
 \expandafter\ifx\csname##1@xy@pdf\endcsname\relax
 \DN@{\defaultinstallpdf@{##1}}}%
 \xydriversselected@@
 \else \DN@##1{}\fi\fi \next@ }
\xydef@\defaultinstallpdf@#1#2{%
 \xywarning@{no driver specified, using #1 }%
 \xyrequire{#1}\csname #1@xy@pdf\endcsname{}}
\xydef@\null@xy@pdf{\installxypdf@}
\xydefcsname@{shape [!...]}#1{%
 \expandafter\ifx\csname xypdf-sloaded\endcsname\empty \DN@{\xyPDFescapestyle@{#1}@@}%
 \else\ifxyPDFshapes@\DN@{\xyPDFshapechar@{#1}@@}%
 \else \DN@{\xyPDFcharwarning@}\fi\fi \next@ }
\xydefcsname@{shape [pdfxy]}{\ifxyPDFshapes@\DN@{\xyPDFpdfxy@}%
 \else \DN@{\xyPDFcharwarning@}\fi \next@ }
\xydef@\xyPDFpdfxy@{%
 \setboxz@h{\dimen@=\L@p \advance\dimen@-\R@p
 \dimen@ii=-\U@p \raise\dimen@ii\hbox to\z@{%
 \kern\dimen@\xyPDFcurrpt@\kern-\dimen@}\boxz@}}%
\xydef@\xyPDFcurrpt@{\ifxyPDFshapes@\expandafter\xyPDFcurrpt@@\fi}
\xydef@\xyPDFcurrpt@@@{\PDFspecial@@{xyi}\PDFraw@@{userdict begin xyx end}}%%%%<<<<<--- here
\ifx\undefined\xyPDFcurrpt@@ \xylet@\xyPDFcurrpt@@=\xyPDFcurrpt@@@ \fi
\xywarnifdefined\xyPDFshapechar@
\xywarnifdefined\xyPDFsplitshape@
{\xyuncatcodes \catcode`@=11
 \gdef\xyPDFshapechar@#1@@{\xyPDFsplitshape@#1<><>@@}%
 \gdef\xyPDFsplitshape@#1<>#2<>#3@@{\xyPDFsplitPDF@{#1}{#2}}}
\xydef@\xyPDFrawA@#1{\expandafter\xyPDFrawAA@ #1{}{}}%
\xydef@\xyPDFrawAA@#1#2{\PDFraw@@{ #1 #2}\PDFmessage{ #1 #2 }}%
\xydef@\xyPDFrawZ@#1{\PDFraw@@{ #1}\PDFmessage{ #1 }}%
\xydef@\modPDFboxz@{%
 \expandafter\DN@\expandafter{\xyPDFpre@{}}\ifx\next@\empty\else
 \setboxz@h{\expandafter\xyPDFrawA@\expandafter{\xyPDFpre@{}}\boxz@
 \expandafter\xyPDFrawZ@\expandafter{\xyPDFpost@}}\DN@{}\fi}%
\xydef@\modPDFdrop@{%
 \expandafter\DNii@\expandafter{%
 \expandafter\xyPDFrawA@\expandafter{\xyPDFpre@{}}}%
 \DN@##1{\expandafter\def\expandafter\tmp@\expandafter{\nextii@ ##1}}%
 \expandafter\next@\expandafter{\Drop@@}%
 \expandafter\DNii@\expandafter{%
 \expandafter\xyPDFrawZ@\expandafter{\xyPDFpost@}}%
 \DN@##1{\expandafter\def\expandafter\Drop@@\expandafter{\tmp@ ##1}}%
 \expandafter\next@\expandafter{\nextii@}}%
\xydef@\modPDFconnect@{%
 \expandafter\DNii@\expandafter{%
 \expandafter\xyPDFrawA@\expandafter{\xyPDFpre@{}}}%
 \DN@##1{\expandafter\def\expandafter\tmp@\expandafter{\nextii@ ##1}}%
 \expandafter\next@\expandafter{\Connect@@}%
 \expandafter\DNii@\expandafter{%
 \expandafter\xyPDFrawZ@\expandafter{\xyPDFpost@}}%
 \DN@##1{\expandafter\def\expandafter\Connect@@\expandafter{\tmp@ ##1}}%
 \expandafter\next@\expandafter{\nextii@}}%
\xydef@\xyPDFpre@{{}{}}
\xydef@\xyPDFpost@{}
\xydef@\PDFmessage@#1{\W@{PDF: #1}}
\xydef@\PDFignore@#1{}%
\xydef@\showPDFmessages{\let\PDFmessage=\PDFmessage@}
\xydef@\hidePDFmessages{\let\PDFmessage=\PDFignore@}
\xylet@\PDFtracing=\showPDFmessages
\hidePDFmessages
\xydef@\PDFmacro@#1{\PDFmacro@@{#1}\PDFmessage{#1}}
\xydef@\includeXYPDFdict@{\relax}
\xydef@\xyPDFdictknown@{}
\xywarnifdefined\obeyoutlines@
{\catcode`\^^M=\active%
 \gdef\obeyoutlines@{\catcode`\^^M=\active \def^^M{^^J}%
 \newlinechar=`\^^J\obeyspaces}}
\xynew@{if}\ifxyPDFshapes@ \xyPDFshapes@true
\xydef@\xyPDFcharwarning@@{\xyPDFcharmessage@
 \gdef\xyPDFcharwarning@@{\xyPDFcharmessage@
 \xywarning@{...no further PDF warnings will be given}%
 \global\let\xyPDFcharwarning@@=\relax }}
\xydef@\xyPDFcharmessage@{\xywarning@{%
 the current <driver> does not fully support PDF effects}}%
\xydef@\newxyshape#1#2#3{%
 \DN@{#3}\ifx\next@\empty
 \xydefcsname@{shape [#1]}{\csname xyshape@#1@\endcsname}%
 \else \expandafter\def\csname shape [#1]\endcsname{%
 \csname xyshape@#1@\endcsname}\fi
 \DN@{#2}\ifx\next@\empty
 \expandafter\def\csname xyshape@#1@\endcsname{%
 \xyundefinedEffect@{#1}{}@@}%
 \else \expandafter\def\csname xyshape@#1@\endcsname{#2}\fi }
\xydef@\xyundefinedEffect@#1#2@@{%
 \xywarning@{The #1 #2 effect is not implemented with the current driver}}%
\xydef@\newxyPDFshape#1#2{%
 \expandafter\DN@\expandafter{\csname shape [#1]\endcsname}%
 \DNii@{\relax}\ifx\next@\nextii@ \newxyshape{#1}{}\relax\fi
 \expandafter\DNii@\expandafter{\csname xyPDFshape@#1@\endcsname}%
 \expandafter\def\nextii@{#2}%
 \ifx\nextii@\empty\expandafter\def\next@{\xyPDFnotimplemented@@`#1'@@}%
 \else
 \edef\tmp@{\noexpand\let\expandafter\noexpand\next@
 \expandafter\noexpand\nextii@}%
 \expandafter\tmp@\fi }
\xydef@\xyPDFnotimplemented@@#1@@{%
 \xywarning@{This PostScript effect is not implemented yet}}%
\xydef@\xyPDFnotfinished@@{%
 \xywarning@{This effect is not reliable yet; box sizes may be wrong}}%
\installxypdf@
\endinput


==> xypdftex.tex <==
%auto-ignore
%this ensures the arxiv doesn't try to start TeXing here.
%% xypdftex.tex from $Id: xypdftex.doc,v $
%%
%% Xy-pic ``pdf-TeX'' driver interface option.
%% Copyright (c) 1999-1999 Ross Moore <ross@mpce.mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-1999 Kristoffer H. Rose <krisrose@brics.dk>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, write to the Free Software Foundation, Inc.,
%% 675 Mass Ave, Cambridge, MA 02139, USA.
%%
\ifx\xyloaded\undefined \input xy \fi
\xyprovide{pdftex}{pdf-TeX driver}{\stripRCS$Revision: 3.8 $}%
 {Ross Moore}{ross@mpce.mq.edu.au}%
 {Mathematics Department, Macquarie University, NSW~2109, Australia}
\xydef@\pdfTeX@@#1{\dvimessage@{pdf-TeX}{#1}}
\newdriver{%
 \xyaddsupport{color}\pdftexColor@@
 \xyaddsupport{crayon}\pdftexCrayon@@
% \xyaddsupport{pdf}\pdftexPDF@@
% \xyaddsupport{rotate}\pdftexRotate@@
 \xyaddsupport{line}\pdftexLine@@
% \xyaddsupport{frame}\pdftexFrames@@
% \xyaddsupport{tile}\pdftexTiles@@
 \xyaddsupport{cmtip}\relax
}
%\xydef@\pdfTeXcolor@push#1{\special{pdfcolor push}\special{pdfcolor #1}}
\xydef@\pdfTeXcolor@push#1{\edef\pdfsaved@color{\pdfcurrent@color}%
 \def\pdfcurrent@color{#1}\special{#1}}%%%<<<<<<--- WRONG !
\xydef@\pdfTeXcolor@pop{\let\pdfcurrent@color\pdfsaved@color
 \expandafter\special\expandafter{\pdfsaved@color}}
\xydef@\pdfTeXcolours@{\pdftexPDFtypes@
% \let\xylocalColor@=\xystackcolor@
% \let\xycolor@push=\pdfTeXcolor@push
% \let\xycolor@pop=\pdfTeXcolor@pop
 \def\xycolor@{\xycolor@@}%
 \expandafter\ifx\csname xypdf-pdfloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xypdf-c}{\xydrivernoload@{pdf-c}}%
 \if@pdf@known\installPDFcolor@ }\else\DN@{}\fi \next@
 \ifx\xycolor@@\xyNoColor@ \let\xycolor@@=\xycolor@raw@@\fi
 \ifx\xycrayolaloaded\empty \DN@{\xystandardcolors@\pdftexCrayon@@{}}%
 \else\let\next@=\xystandardcolors@ \fi \next@
 \let\xycolorwarning@=\relax \pdfTeX@@{color}%
 \let\pdftexColor@@=\relax
 \let\UnloadColor@@=\NopdfTeXcolor@
 }
\xydef@\pdftexColor@@{\pdfTeXcolours@}
\xydef@\NopdfTeXcolor@{%
 \let\xylocalColor@=\xyNoColor@@
 \let\xycolor@=\xyNoColor@
 \let\xycolorwarning@=\xycolorwarning@@
 \let\pdftexColor@@=\pdfTeXcolours@
 \let\UnloadColor@@=\UnloadColor@
 }
\xydef@\pdftexCrayon@@{\pdftexColor@@\pdftexCrayon@}
\xydef@\pdftexCrayon@{\installCrayolaColors@}%
\xydef@\pdftexPDF@@{\if@pdf@known\pdftexPDF@}
\xydef@\pdftexPDFunload@{\if@pdf@known\UnloadPDF@
 \let\UnloadPDF@@=\UnloadPDF@
 \let\pdftexPDF@@=\pdftexPDF@ }
\xydef@\pdftexPDFtypes@{%
 \xyinputorelse@{xypdfpdf}{\xydrivernoload@{pdfpdf}}%
 \ifx\PDFspecial@@\pdfTeXspecial@\else
 \let\PDFspecial@@=\pdfTeXspecial@
 \let\PDFmacro@@=\pdfTeXmacro@
 \let\PDFdict@@=\pdfTeXdict@
 \let\PDFraw@@=\pdfTeXraw@
 \let\PDFinclude@@=\pdfTeXinclude@
 \let\PDFspecialdict@@=\pdfTeXspecialDict@
 \let\xyPDFobeylines@@=\obeypdfTeXlines@
 \pdfTeX@@{PDF}%
 \fi \pdftexCurrpt@ }
\xydef@\pdfTeXspecial@#1{\if@pdf@known\firstPDF@@\pdfobj{#1}\pdflastobj}
\xydef@\pdfTeXmacro@#1{\pdfobj{#1}}
\xydef@\pdfTeXdict@#1{\pdfnames{#1}}
\xydef@\pdfTeXspecialDict@#1{\pdfnames{#1}}
\xydef@\pdfTeXinclude@#1{\if@pdf@known\firstPDF@@\special{prePDFfile #1}}
\xydef@\pdfTeXraw@#1{\if@pdf@known\firstPDF@@\pdfliteral{#1}}%
{\catcode`\^^M=\active%
 \gdef\next{\catcode`\^^M=\active \let^^M=\par%
 \let\PDFspecial@@=\pdfTeXdict@ \obeyspaces}}
\xylet@\obeypdfTeXlines@=\next
\xydef@\pdftexCurrpt@{\let\xyPDFcurrpt@@=\pdftexCurrpt@@}%
\xydef@\pdftexCurrpt@@{\PDFspecial@@{xyi}\PDFraw@@{userdict begin xyx end}}%%%%%<<<<<--- here
\xydef@\pdftexPDF@{\pdftexPDFtypes@
 \let\pdftexPDF@@=\relax
 \let\UnloadPDF@@=\pdftexPDFunload@
 \let\installxypdf@@=\relax \if@pdf@known\installxypdf@ }
\xydef@\pdftexRotate@@{\pdftexRotate@}
\xydef@\pdftexRotate@{\pdftexPDFtypes@
 \expandafter\ifx\csname xypdf-pdfloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xypdf-r}{\xydrivernoload@{pdf-r}}%
 \xyRotScale@@ \if@pdf@known\installPDFrotscale@ }%
 \else\DN@{\xydriverfail@{rotations are}\if@pdf@known\UnloadRotate@\relax}\fi
 \next@}
\xydef@\pdftexLine@@{\pdftexLine@}
\xydef@\pdftexLine@{\pdftexPDFtypes@
 \expandafter\ifx\csname xypdf-pdfloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xypdf-l}{\xydrivernoload@{pdf-l}}%
 \if@pdf@known\installPDFline@ }%
 \else\DN@{\xydriverfail@{line-widths are}\if@pdf@known\UnloadLine@\relax}\fi
 \next@ }
\xydef@\pdftexFrames@@{\pdftexFrames@}
\xydef@\pdftexFrames@{\pdftexPDFtypes@
 \expandafter\ifx\csname xypdf-pdfloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xypdf-f}{\xydrivernoload@{pdf-f}}%
 \if@pdf@known\installPDFframes@ }%
 \else\DN@{\xydriverfail@{frames are}\if@pdf@known\UnloadPDFframes@\relax}\fi
 \next@ }
\xydef@\pdftexTiles@@{\pdftexTiles@}
\xydef@\pdftexTiles@{\pdftexPDFtypes@
 \expandafter\ifx\csname xypdf-pdfloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xypdf-t}{\xydrivernoload@{pdf-t}}%
 \if@pdf@known\installPDFpatterns@ \xystandardpatterns@}%
 \else\DN@{\xydriverfail@{Patterns are}\if@pdf@known\UnloadPDFpatterns@\relax}\fi
 \next@ }
\xydef@\if@pdf@known#1{\ifx\undefined#1\else\expandafter#1\fi}
\xyendinput

